Unlocking the Potential of Federated Learning: The Symphony of Dataset Distillation via Deep Generative Latents

Data heterogeneity presents significant challenges for federated learning (FL). Recently, dataset distillation techniques have been introduced, and performed at the client level, to attempt to mitigate some of these challenges. In this paper, we propose a highly efficient FL dataset distillation framework on the server side, significantly reducing both the computational and communication demands on local devices while enhancing the clients' privacy. Unlike previous strategies that perform dataset distillation on local devices and upload synthetic data to the server, our technique enables the server to leverage prior knowledge from pre-trained deep generative models to synthesize essential data representations from a heterogeneous model architecture. This process allows local devices to train smaller surrogate models while enabling the training of a larger global model on the server, effectively minimizing resource utilization. We substantiate our claim with a theoretical analysis, demonstrating the asymptotic resemblance of the process to the hypothetical ideal of completely centralized training on a heterogeneous dataset. Empirical evidence from our comprehensive experiments indicates our method's superiority, delivering an accuracy enhancement of up to 40% over non-dataset-distillation techniques in highly heterogeneous FL contexts, and surpassing existing dataset-distillation methods by 18%. In addition to the high accuracy, our framework converges faster than the baselines because rather than the server trains on several sets of heterogeneous data distributions, it trains on a multi-modal distribution. Our code is available at https://github.com/FedDG23/FedDG-main.git

==> Supmat.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary

The supplementary material is organized as follows: %Section~\ref{prelim} presents preliminaries; 
in Subsection~\ref{exp:sumpat} additional experiments are provided to compare the performance of FedDGM with the state-of-the-art on high resolution datasets such as ImageNet. This Section further,  presents an ablation study on the impact of different local training epochs on the performance of FedDGM; Section~\ref{sec:related-work} presents the related work to this paper; Section~\ref{dataset-specific} clarifies the subsets of the ImageNet dataset that are used in this paper; Section~\ref{broader-impact} discusses broader impact and limitations; Section~\ref{ethical} presents the ethical considerations
and finally, Section~\ref{conclusion} concludes the paper.

\normalsize

\section{Experiment}\label{exp:sumpat}

\subsection{Performance Comparison on High-resolution Datasets.} \label{exp:supmat:heterogeneity}
This subsection complements subsection~\ref{exp:performance} of the main paper. In this section, we present additional experimental results that explore the correlation between performance improvement and the degree of statistical data heterogeneity. Our objective is to scrutinize whether the conclusions drawn from CIFAR-10 hold true for other high-resolution datasets, specifically subsets of ImageNet.


The reported results in Table~\ref{tab:imfruit_niid} demonstrate a significant improvement achieved by \alg{} compared to the state-of-the-art. \alg{}  led to a remarkable improvement of $15\%$, and $4\%$ over FedDM for the most ($\alpha=0.01$) and the least ($\alpha=0.9$) heterogeneous setting. These findings further reinforce the claim that \emph{greater data heterogeneity correlates with amplified performance improvement in the global model trained through our dataset distillation method \alg{} }. For a concise comprehension of the key findings within these extensive tables, we have summarized the average accuracy in the last column of Table~\ref{tab:imfruit_niid} in Fig.~\ref{fig:avg_iid_fruit}.


 



\footnotesize{
\begin{table}[htbp]
\footnotesize
\begin{center}
\footnotesize
\caption{\small{Impact of different values of $\alpha$ on the ImageFruit dataset.}}

\vspace{-1mm}
% \begin{table}[H]
    \color{black}
    % \caption{Results for \textbf{Average Final Local Accuracy} for Non-IID $(20\%)$}
    \label{tab:imfruit_niid}
    \centering
 \resizebox{\columnwidth}{!}{
\begin{tabular}{ll|lllll}
            \toprule
$\alpha$     &Algorithm & ConvNet  & ResNet18   & ResNet34  & Average\\
            \midrule
            &FedAvg & 43.9$_{\pm 0.3}$& 35.1$_{\pm 0.8}$ & 41.8$_{\pm 0.4}$ & 40.3$_{\pm 0.5}$ \\

            &FedProx  & 48.5$_{\pm 0.9}$& 37.1$_{\pm 0.9}$ & 38.9$_{\pm 1.4}$ & 41.5$_{\pm 1.1}$ \\

0.9        &FedNova  & 46.8$_{\pm 0.7}$& 37.6$_{\pm 0.9}$ & 42.2$_{\pm 1.1}$ & 42.2$_{\pm 0.9}$ \\

            &FedDM  & 49.7$_{\pm 0.2}$& 51.7$_{\pm 0.5}$ & 56.7$_{\pm 0.9}$ & 52.7$_{\pm 0.5}$ \\

            &\alg{} & 54.6$_{\pm 0.9}$& 55.7$_{\pm 0.7}$ & 59.1$_{\pm 0.8}$ & 56.5$_{\pm 0.8}$ \\

            \midrule
            
            &FedAvg & 42.7$_{\pm 1.9}$& 36.2$_{\pm 1.4}$ &39.5$_{\pm 2.6}$ &39.5$_{\pm 2.0}$ \\

            &FedProx  & 43.9$_{\pm 0.2}$& 34.7$_{\pm 1.8}$ &42.4$_{\pm 3.3}$ &40.4$_{\pm 1.8}$ \\

0.5         &FedNova  & 45.7$_{\pm 1.2}$& 35.0$_{\pm 0.6}$ &39.1$_{\pm 1.0}$ &40.0$_{\pm 1.0}$ \\

            &FedDM  & 45.7$_{\pm 1.7}$& 49.7$_{\pm 0.2}$ & 53.7$_{\pm 1.5}$ &49.7$_{\pm 1.1}$ \\

            &\alg{} & 54.5$_{\pm 1.5}$& 55.1$_{\pm 0.7}$ &58.9$_{\pm 0.4}$ &56.2$_{\pm 0.8}$ \\
         
            \midrule 

            &FedAvg & 42.1$_{\pm 1.5}$& 33.4$_{\pm 2.2}$ & 38.0$_{\pm 1.5}$ & 37.8$_{\pm 1.7}$ \\

            &FedProx  & 39.8$_{\pm 1.2}$& 32.1$_{\pm 2.2}$ & 34.2$_{\pm 1.3}$ & 35.4$_{\pm 1.6}$ \\

0.1        &FedNova  & 40.6$_{\pm 1.0}$& 31.5$_{\pm 1.6}$ & 34.9$_{\pm 2.5}$ & 35.6$_{\pm 1.7}$ \\

            &FedDM  & 42.3$_{\pm 1.2}$& 45.1$_{\pm 0.7}$ & 48.7$_{\pm 0.7}$ & 45.3$_{\pm 0.8}$ \\

            &\alg{} & 51.3$_{\pm 0.6}$& 51.6$_{\pm 1.8}$ & 59.1$_{\pm 1.5}$ & 54.0$_{\pm 1.3}$ \\               
    
 \midrule

            &FedAvg & 23.7$_{\pm 0.1}$& 17.7$_{\pm 0.5}$ & 16.7$_{\pm 0.9}$ & 19.3$_{\pm 0.5}$ \\

            &FedProx  & 21.8$_{\pm 1.7}$& 16.3$_{\pm 0.3}$ & 17.7$_{\pm 0.8}$ & 18.6$_{\pm 0.9}$ \\

0.01        &FedNova  & 22.3$_{\pm 1.5}$& 20.0$_{\pm 1.1}$ &17.1$_{\pm 0.6}$ &19.8$_{\pm 1.1}$ \\

            &FedDM  & 32.9$_{\pm 1.5}$& 37.3$_{\pm 0.9}$ & 34.5$_{\pm 0.7}$ & 34.9$_{\pm 1.0}$ \\

            &\alg{} & 44.9$_{\pm 1.4}$& 48.5$_{\pm 0.7}$ & 55.1$_{\pm 0.2}$ & 49.5$_{\pm 0.8}$ \\
                   
 

\midrule
        \end{tabular}
     }
% \end{table}
\end{center}
  %\vspace{-4mm}
\end{table}




\begin{figure}[ht]
  \begin{minipage}{\columnwidth}
    \centering
  % \includegraphics[width=.99\columnwidth]{figs/ImageNet-diff_subset.eps}
  \includegraphics[width=.99\columnwidth]{figs/diff_alpha_fruit.eps}
    \vspace{-4mm}
    \caption{Impact of different $\alpha$ on the average accuracy across global models with different architectures on ImageFruit.}
    \label{fig:avg_iid_fruit}
  \end{minipage}\\[1em]
    \vspace{-4mm}
\end{figure}

\iffalse
\begin{figure}[ht]
  \begin{minipage}{\columnwidth}
    \centering
  % \includegraphics[width=.99\columnwidth]{figs/ImageNet-diff_subset.eps}
  \includegraphics[width=.99\columnwidth]{figs/ImageNet-diff_subset.pdf}
    \vspace{-2mm}
    \caption{Illustrations of distilled data generated from different ImageNet subsets. Each row of images corresponds to a subset, from top to bottom: ImageMeow, ImageWoof, ImageFruit, ImageFood, and ImageMisc.}
    \label{fig:imagenet_diff_subsets}
  \end{minipage}\\[1em]
    \vspace{-4mm}
\end{figure}
\fi


\normalsize

 % \noindent \textbf{Impact of Different Local Training Epochs.} 
\subsection{Impact of Different Local Training Epochs} 
Fig.~\ref{fig:diff_localepoch} shows the results when clients train local surrogate models with different numbers of local epochs $T_l$ using their local real data. Interestingly, we can observe that as the number of local epochs increases, the mean accuracy of global models does not consistently improve. The global model's performance is best when the number of local epochs is set to 20, and deviating from this value, either higher or lower, results in a relatively small decrease in performance.

When the number of local epochs is small, local surrogate models are updated less frequently, leading to a slower convergence rate in the overall FL training process. On the other hand, when the number of local epochs increases, it introduces a larger gap between the post-training local surrogate model parameters $\theta_m^{(t+1)}$ and the global model parameters $\theta_g^{(t)}$ from the previous communication round. This increased gap makes it more challenging for the server to apply matching training trajectories to distill data. As a result, when the distillation step $T_d$ remains constant, a larger number of local epochs can actually lead to a decrease in the quality of the distilled data.

\begin{figure}[ht]
  \begin{minipage}{\columnwidth}
    \centering
  % \includegraphics[width=.99\columnwidth]{figs/ImageNet-diff_subset.eps}
  \includegraphics[width=.99\columnwidth]{figs/diff_localepoch.eps}
  \vspace{-4mm}
    \caption{\footnotesize \textbf{Test accuracy experiences a slight decrease when utilizing very high or very low local epochs.} Impact of different numbers of local epochs. When the number of local epochs is 20, \alg{} achieves its best cross-architecture performance. Deviating from this value, whether greater or lesser than 20, results in a slight decrease in test accuracy. }
    % By default, we train the local model for 20 local epochs.}
    \label{fig:diff_localepoch}
  \end{minipage}\\[1em]
  \vspace{-6mm}
\end{figure}





\normalsize

\input{Related-Work}

\section{Dataset Specifications} \label{dataset-specific}
Our subsets are derived from ImageNet ILSVRC2012. For each subset, we select 10 classes with similar features from the 1000 classes in ImageNet. The training set of each ImageNet subset is composed of all the training images belonging to these 10 classes, while the validation set consists of all the validation images from the same classes. Table~\ref{tab:cate_subset} shows the specific categories that make up each subset.


\section{Broader Impacts} \label{broader-impact}
The primary objective of dataset distillation is to alleviate the storage and computational resource requirements for training deep neural networks. This need is particularly critical in the era of foundational models. The goal of dataset distillation aligns with advancing environmental sustainability efforts. In this context, the introduced FedDGM method notably diminishes the resource demands associated with the training process compared to conventional training. Our aspiration is that this contribution encourages the computer vision community to focus more on pragmatic dataset distillation approaches, fostering the sustainable development of society.


\section{Ethical Considerations} \label{ethical}

This work does not involve any immediate ethical concerns. Our experiments utilize the publicly accessible ImageNet and CIFAR-10 datasets. 

% \footnotesize{
\begin{table*}[htbp]
% \footnotesize
\begin{center}
\footnotesize
\caption{\small{Categories in ImageNet subsets}}

\vspace{-1mm}
% \begin{table}[H]
    \color{black}
    \label{tab:cate_subset}
    \centering
 \resizebox{\textwidth}{!}{

\begin{tabular}{l|cccccccccc}
\toprule
Subset  & 0                                                            & 1                                                        & 2                                                     & 3                                                     & 4                                                      & 5                                                          & 6                                                             & 7                                                        & 8                                                          & 9                                                          \\ \midrule
ImMeow  & \begin{tabular}[c]{@{}c@{}}Tabby\\ Cat\end{tabular}          & \begin{tabular}[c]{@{}c@{}}Bengal\\ Cat\end{tabular}     & \begin{tabular}[c]{@{}c@{}}Persian\\ Cat\end{tabular} & \begin{tabular}[c]{@{}c@{}}Siamese\\ Cat\end{tabular} & \begin{tabular}[c]{@{}c@{}}Egyptian\\ Cat\end{tabular} & Lion                                                       & Tiger                                                         & Jaguar                                                   & \begin{tabular}[c]{@{}c@{}}Snow\\ Leopard\end{tabular}     & Lynx                                                       \\ \midrule
ImWoof  & \begin{tabular}[c]{@{}c@{}}Australian\\ Terrier\end{tabular} & \begin{tabular}[c]{@{}c@{}}Border\\ Terrier\end{tabular} & Samoyed                                               & Beagle                                                & Shih-Tzu                                               & \begin{tabular}[c]{@{}c@{}}English\\ Foxhound\end{tabular} & \begin{tabular}[c]{@{}c@{}}Rhodesian\\ Ridgeback\end{tabular} & Dingo                                                    & \begin{tabular}[c]{@{}c@{}}Golden\\ Retriever\end{tabular} & \begin{tabular}[c]{@{}c@{}}English\\ Sheepdog\end{tabular} \\ \midrule
ImFruit & Pineapple                                                    & Banana                                                   & Strawberry                                            & Orange                                                & Lemon                                                  & Pomegranate                                                & Fig                                                           & \begin{tabular}[c]{@{}c@{}}Bell\\ Pepper\end{tabular}    & Cucumber                                                   & \begin{tabular}[c]{@{}c@{}}Green\\ Apple\end{tabular}      \\ \midrule
ImFood  & Cheeseburger                                                 & Hot-dog                                                   & Pretzel                                               & Pizza                                                 & French Loaf                                            & Ice-cream                                                  & Guacamole                                                     & Carbonara                                                & Bagel                                                      & Trifle                                                     \\ \midrule
ImMisc  & Bubble                                                       & \begin{tabular}[c]{@{}c@{}}Piggy\\ Bank\end{tabular}     & Stoplight                                             & Coil                                                  & Kimono                                                 & Cello                                                      & \begin{tabular}[c]{@{}c@{}}Combination\\ Lock\end{tabular}    & \begin{tabular}[c]{@{}c@{}}Triumphal\\ Arch\end{tabular} & Fountain                                                   & \begin{tabular}[c]{@{}c@{}}Spaghetti\\ Squash\end{tabular} \\ \midrule
\end{tabular}}
% \end{table}
\end{center}
  %\vspace{-4mm}
\end{table*}

\input{Conclusion}

